Modelling Wind Turbines via Actuator Lines in High-Order h/p Solvers

This paper compares two actuator line methodologies for modelling wind turbines employing high-order h/p solvers and large-eddy simulations. The methods combine the accuracy of high-order solvers (in this work the maximum order is 6) with the computational efficiency of actuator lines to capture the aerodynamic effects of wind turbine blades. Comparisons with experiments validate the actuator line methodologies. We explore the effects of the polynomial order and the smoothing parameter associated with the Gaussian regularization function, and use them to blend the actuator line forcing in the high-order computational mesh, to show that both parameters influence the distribution of forces along the blades and the turbine wake. The greatest impact is obtained when the polynomial order is increased, allowing one to better capture the physics without requiring new meshes. When comparing the actuator line methodologies, we show the advantages of performing weighted sums, over element averages, to compute the blade velocities and forces in high-order solvers. For low-order simulations (low polynomial orders), both methods provide similar results, but as the polynomial order is increased, the weighted sum method shows smoother thrust/torque distributions and better wake resolution. Furthermore, cell averaging introduces nonphysical oscillations when increasing the polynomial order beyond 3 (4th order accuracy).

==> bibliography.tex <==
\begin{thebibliography}

\bibitem{sorensen2015simulation}
Sørensen J.N, Mikkelsen R.F, Henningson D.S, Ivanell S, Sarmast S and Andersen S.J. Simulation of wind turbine wakes using the actuator line technique. Philos. Trans. Royal Soc. A. 2015;373:1-16. http://dx.doi.org/10.1098/rsta.2014.0071
%----------------------------------------------------------------------------------
\bibitem{arabgolarcheh2023}
Arabgolarcheh A, Micallef D, Rezaeiha A and Benini E. Modelling of two tandem floating offshore wind turbines using an actuator line model. Renewable Energy. 2023;216:119067. https://doi.org/10.1016/j.renene.2023.119067
%----------------------------------------------------------------------------------
\bibitem{HORSES_3D}
Ferrer E, Rubio G, Ntoukas G, Laskowski W, Mariño O.A, Colombo S, Mateo-Gabín A, Marbona H, Manrique de Lara F, Huergo D, Manzanero J, Rueda-Ramírez A.M, Kopriva D.A and Valero E. HORSES3D: A high-order discontinuous Galerkin solver for ﬂow simulations and multi-physics applications. Computer Physics Communications. 2023;287:108700. https://doi.org/10.1016/j.cpc.2023.108700
%----------------------------------------------------------------------------------
\bibitem{Tossas_epsilon}
Martínez-Tossas L.A, Churchfield M.J, Meneveau C. Large eddy simulation of wind turbine wakes: detailed comparisons of two codes focusing on effects of numerics and subgrid modeling. J Phys Conf Ser. 2015;625:12024. doi:10.1088/1742-6596/625/1/012024
%----------------------------------------------------------------------------------
\bibitem{Toldborg_epsilon}
Troldborg N, Sørensen J.N, Mikkelsen R.F. Numerical simulations of wake characteristics of a wind turbine in uniform inflow. Wind Energy. 2010;13:86-99. doi:10.1002/we.345
%----------------------------------------------------------------------------------
\bibitem{Datos_experimentales}
Per-Åge Krogstad and Sætran L. Wind Turbine Wake Interactions; Results From Blind Tests. J Phys Conf Ser. 2015;625(1):012043. doi:10.1088/1742-6596/625/1/012043 
%----------------------------------------------------------------------------------
\bibitem{Blind_Test_geometria}
Melheim J.A. "Blind test" Workshop Calculations for a model wind turbine, Department of Energy and Process Engineering, NTNU, 2011
%----------------------------------------------------------------------------------
\bibitem{BEMT}
Schaffarczyk A.P. Introduction to Wind Turbine Aerodynamics. Mechanical Engineering Department, University of Applied Sciences. 2014.
%----------------------------------------------------------------------------------
\bibitem{Datos_numéricos}
Deskos G, Laizet S, Piggott M.D. Turbulence-resolving simulations of wind turbine wakes. Department of Aeronautics, Imperial College London, London. April 2018.
%----------------------------------------------------------------------------------
\bibitem{Tip correction}
Wen Zhong Shen, Robert Mikkelsen, Jens Nørkær Sørensen, Christian Bak. Tip loss corrections for
wind turbine computations. Wiley Interscience, Wind Energy, 2005.

\end{thebibliography}
